Securing External Deeper-than-black-box GPAI Evaluations

This paper examines the critical challenges and potential solutions for conducting secure and effective external evaluations of general-purpose AI (GPAI) models. With the exponential growth in size, capability, reach and accompanying risk of these models, ensuring accountability, safety, and public trust requires frameworks that go beyond traditional black-box methods. The discussion begins with an analysis of the need for deeper-than-black-box evaluations (Section I), emphasizing the importance of understanding model internals to uncover latent risks and ensure compliance with ethical and regulatory standards. Building on this foundation, Section II addresses the security considerations of remote evaluations, outlining the threat landscape, technical solutions, and safeguards necessary to protect both evaluators and proprietary model data. Finally, Section III synthesizes these insights into actionable recommendations and future directions, aiming to establish a robust, scalable, and transparent framework for external assessments in GPAI governance.

==> old_refs.tex <==
\begin{thebibliography}{99}

\bibitem{bengio2025international}
Yoshua Bengio, Sören Mindermann, Daniel Privitera, Tamay Besiroglu, Rishi Bommasani, Stephen Casper, Yejin Choi, Philip Fox, Ben Garfinkel, and Danielle Goldfarb. \textit{International AI Safety Report}. arXiv preprint arXiv:2501.17805, 2025.

\bibitem{mallen2023eliciting}
Alex Mallen, Madeline Brumley, Julia Kharchenko, and Nora Belrose. \textit{Eliciting latent knowledge from quirky language models}. arXiv preprint arXiv:2312.01037, 2023.

\bibitem{burns2022discovering}
Collin Burns, Haotian Ye, Dan Klein, and Jacob Steinhardt. \textit{Discovering latent knowledge in language models without supervision}. arXiv preprint arXiv:2212.03827, 2022.

\bibitem{bucknall2023structured}
Benjamin S. Bucknall and Robert F. Trager. \textit{Structured Access for third-party research on frontier AI models: investigating researcher’s model access requirements}. Oxford Martin School, University of Oxford; Center for the Governance of AI, 2023.

\bibitem{METR-1}
Beth Barnes. \textit{Details about METR's preliminary evaluation of GPT-4o}. Available at \url{https://metr.github.io/autonomy-evals-guide/gpt-4o-report/}, 2024.

\bibitem{meinke2024frontier}
Alexander Meinke, Bronson Schoen, Jérémy Scheurer, Mikita Balesni, Rusheb Shah, and Marius Hobbhahn. \textit{Frontier Models are Capable of In-context Scheming}. arXiv preprint arXiv:2412.04984, 2024.

\bibitem{hubinger2024sleeper}
Evan Hubinger, Carson Denison, Jesse Mu, Mike Lambert, Meg Tong, Monte MacDiarmid, Tamera Lanham, Daniel M. Ziegler, Tim Maxwell, and Newton Cheng. \textit{Sleeper agents: Training deceptive LLMs that persist through safety training}. arXiv preprint arXiv:2401.05566, 2024.

\bibitem{panickssery2023reducing}
Nina Panickssery. \textit{Reducing sycophancy and improving honesty via activation steering}. In AI Alignment Forum, 2023.

\bibitem{Farquhar2024Detecting}
Sebastian Farquhar, Jannik Kossen, Jiatong Han, Muhammed Razzak, Lisa Schut, Shreshth Malik, and Yarin Gal. \textit{Detecting hallucinations in large language models using semantic entropy}. Nature, 615:123--128, 2024. \url{https://www.nature.com/articles/s41586-024-07421-0}.

\bibitem{azaria2023internal}
Amos Azaria and Tom Mitchell. \textit{The internal state of an LLM knows when it's lying}. arXiv preprint arXiv:2304.13734, 2023.

\bibitem{egloff2021attribution}
Florian J. Egloff and Myriam Dunn--Cavelty. \textit{Attribution and knowledge creation assemblages in cybersecurity politics}. Journal of Cybersecurity, 7(1):tyab002, 2021.

\bibitem{elshandidy2021independent}
Tamer Elshandidy, Mohamed Khaled Eldaly, and Magdy Abdel--Kader. \textit{Independent oversight of the auditing profession: A review of the literature}. International Journal of Auditing, 25(2):373--407, 2021.

\bibitem{jaech2024openai}
Aaron Jaech, Adam Kalai, Adam Lerer, Adam Richardson, Ahmed El--Kishky, Aiden Low, Alec Helyar, Aleksander Madry, Alex Beutel, and Alex Carney. \textit{Openai o1 system card}. arXiv preprint arXiv:2412.16720, 2024.

\bibitem{guo2025deepseek}
Daya Guo, Dejian Yang, Haowei Zhang, Junxiao Song, Ruoyu Zhang, Runxin Xu, Qihao Zhu, Shirong Ma, Peiyi Wang, and Xiao Bi. \textit{Deepseek-r1: Incentivizing reasoning capability in LLMs via reinforcement learning}. arXiv preprint arXiv:2501.12948, 2025.

\bibitem{casper2024black}
Stephen Casper, Carson Ezell, Charlotte Siegmann, Noam Kolt, Taylor Lynn Curtis, Benjamin Bucknall, Andreas Haupt, Kevin Wei, Jérémy Scheurer, and Marius Hobbhahn. \textit{Black-box access is insufficient for rigorous AI audits}. In Proceedings of the 2024 ACM Conference on Fairness, Accountability, and Transparency, pages 2254--2272, 2024.

\bibitem{Cunningham2023Sparse}
Hoagy Cunningham, Aidan Ewart, Logan Riggs, Robert Huben, and Lee Sharkey. \textit{Sparse Autoencoders Find Highly Interpretable Features in Language Models}. arXiv preprint arXiv:2309.08600, 2023. \url{https://arxiv.org/abs/2309.08600}.

\bibitem{templeton2024scaling}
Adly Templeton. \textit{Scaling monosemanticity: Extracting interpretable features from Claude 3 sonnet}. Anthropic, 2024.

\bibitem{wehner2023representation}
Jan Wehner. \textit{An Introduction to Representation Engineering -- an activation-based paradigm for controlling LLMs}. AI Alignment Forum, 2023.

\bibitem{Vig2020Causal}
Jesse Vig, Atticus Geiger, Swabha Swayamdipta, Brendan Hoover, Sameer Singh, and Yonatan Belinkov. \textit{Causal Mediation Analysis for Interpreting Neural NLP: The Case of Gender Bias}. arXiv preprint arXiv:2004.12265, 2020. \url{https://arxiv.org/abs/2004.12265}.

\bibitem{Burns2023Steering}
Collin Burns, Haotian Ye, Aaron Klein, and Jacob Steinhardt. \textit{Steering Language Models With Activation Engineering}. arXiv preprint arXiv:2308.10248, 2023. \url{https://arxiv.org/abs/2308.10248}.

\bibitem{arditi2024refusal}
Andy Arditi, Oscar Obeso, Aaquib Syed, Daniel Paleka, Nina Panickssery, Wes Gurnee, and Neel Nanda. \textit{Refusal in language models is mediated by a single direction}. arXiv preprint arXiv:2406.11717, 2024.

\bibitem{Nanda2023Attribution}
Neel Nanda. \textit{Attribution Patching: Activation Patching at Industrial Scale}. Unpublished manuscript, 2023.

\bibitem{goldowsky2023localizing}
Nicholas Goldowsky--Dill, Chris MacLeod, Lucas Sato, and Aryaman Arora. \textit{Localizing model behavior with path patching}. arXiv preprint arXiv:2304.05969, 2023.

\bibitem{Elhage2022Causal}
Nelson Elhage, Neel Nanda, Catherine Olsson, Tom Henighan, Nicholas Joseph, Dario Amodei, Tom Brown, Jack Clark, Ben Mann, and Sam McCandlish. \textit{Causal Scrubbing: A method for rigorously testing interpretability hypotheses}. AI Alignment Forum, 2022.

\bibitem{dunefsky2024transcoders}
Jacob Dunefsky, Philippe Chlenski, and Neel Nanda. \textit{Transcoders Find Interpretable LLM Feature Circuits}. arXiv preprint arXiv:2406.11944, 2024.

\bibitem{Ravfogel2023LEACE}
Shauli Ravfogel, Yanai Elazar, Hila Gonen, and Michael Twiton. \textit{LEACE: Perfect linear concept erasure in closed form}. arXiv preprint arXiv:2306.03819, 2023. \url{https://arxiv.org/abs/2306.03819}.

\bibitem{Rauber2017Foolbox}
Jonas Rauber, Wieland Brendel, and Matthias Bethge. \textit{Foolbox: A Python Toolbox to Create Adversarial Examples that Fool Neural Networks in PyTorch, TensorFlow, and JAX}. GitHub repository, 2017.

\bibitem{croce2020reliable}
Francesco Croce and Matthias Hein. \textit{Reliable evaluation of adversarial robustness with an ensemble of diverse parameter-free attacks}. In International Conference on Machine Learning, pages 2206--2216, 2020.

\bibitem{koh2021wilds}
Pang--Wei Koh, Shiori Sagawa, Henrik Marklund, Sang--Michael Xie, Marvin Zhang, Akshay Balsubramani, Weihua Hu, Michihiro Yasunaga, Richard Lanas Phillips, and Irena Gao. \textit{Wilds: A benchmark of in-the-wild distribution shifts}. In International Conference on Machine Learning, pages 5637--5664, 2021.

\bibitem{OpenAI2023RedTeaming}
OpenAI. \textit{Red Teaming}. Available at \url{https://openai.com/research/red-teaming}, 2023.

\bibitem{ganguli2022red}
Deep Ganguli, Liane Lovitt, Jackson Kernion, Amanda Askell, Yuntao Bai, Saurav Kadavath, Ben Mann, Ethan Perez, Nicholas Schiefer, and Kamal Ndousse. \textit{Red teaming language models to reduce harms: Methods, scaling behaviors, and lessons learned}. arXiv preprint arXiv:2209.07858, 2022.

\bibitem{zhu2023gradient}
Rui Zhu, Di Tang, Siyuan Tang, Guanhong Tao, Shiqing Ma, Xiaofeng Wang, and Haixu Tang. \textit{Gradient shaping: Enhancing backdoor attack against reverse engineering}. arXiv preprint arXiv:2301.12318, 2023.

\bibitem{pan2023asset}
Minzhou Pan, Yi Zeng, Lingjuan Lyu, Xue Lin, and Ruoxi Jia. \textit{ASSET: Robust backdoor data detection across a multiplicity of deep learning paradigms}. In Proceedings of the 32nd USENIX Security Symposium (USENIX Security 23), pages 2725--2742, 2023.

\bibitem{sundararajan2017axiomatic}
Mukund Sundararajan, Ankur Taly, and Qiqi Yan. \textit{Axiomatic attribution for deep networks}. In International Conference on Machine Learning, pages 3319--3328, 2017.

\bibitem{smilkov2017smoothgrad}
Daniel Smilkov, Nikhil Thorat, Been Kim, Fernanda Viégas, and Martin Wattenberg. \textit{Smoothgrad: removing noise by adding noise}. arXiv preprint arXiv:1706.03825, 2017.

\bibitem{hu2022membership}
Hongsheng Hu, Zoran Salcic, Lichao Sun, Gillian Dobbie, Philip S. Yu, and Xuyun Zhang. \textit{Membership inference attacks on machine learning: A survey}. ACM Computing Surveys (CSUR), 54(11):1--37, 2022.

\bibitem{zhou2024model}
Zhanke Zhou, Jianing Zhu, Fengfei Yu, Xuan Li, Xiong Peng, Tongliang Liu, and Bo Han. \textit{Model Inversion Attacks: A Survey of Approaches and Countermeasures}. arXiv preprint arXiv:2411.10023, 2024.

\bibitem{dutta2024think}
Subhabrata Dutta, Joykirat Singh, Soumen Chakrabarti, and Tanmoy Chakraborty. \textit{How to think step-by-step: A mechanistic understanding of chain-of-thought reasoning}. arXiv preprint arXiv:2402.18312, 2024.

\bibitem{nevo2024securing}
SELLA NEVO, DAN LAHAV, AJAY KARPUR, YOGEV BAR--ON, HENRY ALEXANDER BRADLEY, and JEFF ALSTOTT. \textit{Securing AI Model Weights}. 2024.

\bibitem{dutta2023spy}
Sankha Baran Dutta, Hoda Naghibijouybari, Arjun Gupta, Nael Abu--Ghazaleh, Andres Marquez, and Kevin Barker. \textit{Spy in the GPU-box: Covert and Side Channel Attacks on Multi-GPU Systems}. In Proceedings of the 50th Annual International Symposium on Computer Architecture (ISCA '23), 2023. doi:10.1145/3579371.3589080.

\bibitem{Naghibijouybari21side}
Hoda Naghibijouybari, Ajaya Neupane, Zhiyun Qian, and Nael B. Abu--Ghazaleh. \textit{Side Channel Attacks on GPUs}. IEEE Trans. Dependable Secur. Comput., 18(4):1950--1961, 2021. doi:10.1109/TDSC.2019.2944624.

\bibitem{trask2020beyond}
Andrew Trask, Emma Bluemke, Teddy Collins, Ben Garfinkel, Claudia Ghezzou Cuervas--Mons, Iason Gabriel, Allan Dafoe, and William Isaac. \textit{Beyond privacy trade-offs with structured transparency}. arXiv preprint arXiv:2012.08347, 2020.

\bibitem{tramer2022position}
Florian Tramèr, Gautam Kamath, and Nicholas Carlini. \textit{Position: Considerations for Differentially Private Learning with Large-Scale Public Pretraining}. In Forty-first International Conference on Machine Learning, 2022.

\bibitem{gamiz2025challenges}
Idoia Gamiz, Cristina Regueiro, Oscar Lage, Eduardo Jacob, and Jasone Astorga. \textit{Challenges and future research directions in secure multi-party computation for resource-constrained devices and large-scale computations}. International Journal of Information Security, 24(1):1--29, 2025.

\bibitem{islam2024confidential}
Md Shihabul Islam. \textit{Confidential Computing with Trusted Execution Environments}. PhD thesis, 2024.

\bibitem{tramer2018slalom}
Florian Tramèr and Dan Boneh. \textit{Slalom: Fast, verifiable and private execution of neural networks in trusted hardware}. arXiv preprint arXiv:1806.03287, 2018.

\bibitem{carlini2024stealing}
Nicholas Carlini, Daniel Paleka, Krishnamurthy Dj Dvijotham, Thomas Steinke, Jonathan Hayase, A Feder Cooper, Katherine Lee, Matthew Jagielski, Milad Nasr, and Arthur Conmy. \textit{Stealing part of a production language model}. arXiv preprint arXiv:2403.06634, 2024.

\bibitem{dwork2014algorithmic}
Cynthia Dwork and Aaron Roth. \textit{The algorithmic foundations of differential privacy}. Foundations and Trends in Theoretical Computer Science, 9(3--4):211--407, 2014.

\bibitem{Ronis2024ZeroKnowledge}
Jared Ronis. \textit{Don't Trust When You Can Verify: A Primer on Zero-Knowledge Proofs}. February 2024. \url{https://www.wilsoncenter.org/article/dont-trust-when-you-can-verify-primer-zero-knowledge-proofs}.

\bibitem{waiwitlikhit2024trustless}
Suppakit Waiwitlikhit, Ion Stoica, Yi Sun, Tatsunori Hashimoto, and Daniel Kang. \textit{Trustless Audits without Revealing Data or Models}. arXiv preprint arXiv:2404.04500, 2024.

\bibitem{shi2022auditem}
Zeshun Shi, Jeroen Bergers, Ken Korsmit, and Zhiming Zhao. \textit{AUDITEM: toward an automated and efficient data integrity verification model using blockchain}. arXiv preprint arXiv:2207.00370, 2022.

\bibitem{feng2025blockchain}
Shuai Feng, Lunzhi Deng, Yan Gao, Yaying Wu, and Jian Wen. \textit{Blockchain-based remote data integrity auditing scheme with deduplication mechanism}. Cluster Computing, 28(1):33, 2025.

\bibitem{octaviani2021effect}
Dwirezki Octaviani and Kurnia Ekasari. \textit{The Effect of Due Professional Care, Integrity, Confidentiality, and Independence on Audit Quality}. In Proceedings of the 2nd Annual Management, Business and Economic Conference (AMBEC 2020), pages 106--110, 2021.

\bibitem{asa2006auditing}
Compiled Auditing Standard. \textit{Auditing standard ASA 210 terms of audit engagements}. Auditing, Assurance Standards Board Melbourne, Australia, 2006.

\bibitem{oueslati2025external}
Amin Oueslati. \textit{External Assessments in the EU Code of Practice for GPAI Model Providers}. The Future Society, 2025.

\bibitem{trager2025who}
Lara Thurnherr, Robert Trager, Amin Oueslati, Christoph Winter, Cliodhna Ní Ghuidhir, Joe O'Brien, Jun Shern Chan, Lorenzo Pacchiardi, Anka Reuel, Merlin Stein, and Oliver Guest. \textit{Who Should Develop Which AI Evaluations?} Oxford Martin School, University of Oxford and Center for the Governance of AI, 2025.

\end{thebibliography}
